On the Analysis of a Multipartite Entanglement Distribution Switch

We study a quantum switch that distributes maximally entangled multipartite states to sets of users. The entanglement switching process requires two steps: first, each user attempts to generate bipartite entanglement between itself and the switch; and second, the switch performs local operations and a measurement to create multipartite entanglement for a set of users. In this work, we study a simple variant of this system, wherein the switch has infinite memory and the links that connect the users to the switch are identical. Further, we assume that all quantum states, if generated successfully, have perfect fidelity and that decoherence is negligible. This problem formulation is of interest to several distributed quantum applications, while the technical aspects of this work result in new contributions within queueing theory. Via extensive use of Lyapunov functions, we derive necessary and sufficient conditions for the stability of the system and closed-form expressions for the switch capacity and the expected number of qubits in memory.

==> Delay.tex <==
%%!TEX PS-program = pdflatexmk
%%!TEX root = main.tex

Each entanglement swapping operation \cite{zukowski1993event} induces a communication delay between the central node  and the $n$  users involved in the operation.
%This delay is due to the transmission to the users of the measurement results performed at the switch. 
If we denote by $t_j$ the time when the $j$-th swapping operation takes place then, if successful, the resulting end-to-end entanglement between the $n$ involved users 
will be completed at time $t_j+\Delta$, where $\Delta$ is a finite nonnegative constant equal to the time needed for all $n$ users to receive the result of the measurement performed at the central
node. 

In this setting, the capacity is given by $\lim_{j}\frac{j}{t_j+\Delta}=\lim_{j}\frac{j}{t_j}\times \frac{t_j}{t_j+\Delta}= C\times \lim_{t} \frac{t_j}{t_j+\Delta}
=C$ a.s. since $t_j\to\infty$ as $j\to\infty$. In other words, the capacity remains unchanged by the introduction of the constant delay $\Delta$.  The expected number of
Bell pairs stored at the central node is also unchanged since, by definition, it focuses on the number of Bell pairs {\em before} a swap.

We show below that the stability condition $n<k$ still holds provided that $\Delta<\frac{1}{\mu (k-(n-1))}$. %In practice $\mu\ll 1/\Delta$. 

We define a {\em swapping period}  as the time period  that elapses between the time instant when a swapping operation starts whenever there are no swapping operations in
progress and the next time instant where there is 
no swapping operation in progress.  Note that if $[t_j,t'_j)$ denotes the  $j$-th swapping period then $t'_j$ is not necessarily equal to $t_j+\Delta$ as $t'_j$ will be larger than $t_j+\Delta$  if at least one swapping operation is  initialized  in $(t_j,t_j+\Delta)$.

Under the assumption that $\Delta<\frac{1}{\mu (k-(n-1))}$ it can be shown \textcolor{blue}{TBD -- proof uses Tak\`acs' argument} that the duration of a  swapping period is almost surely (a.s.) finite, so that the sequence $\{t'_j\}$ is a.s. increasing, with the consequence that $\lim_j t'_j$ exists a.s. This limit is infinite as  $t_{j+1}-t'_j$ is stochastically larger than an exponential r.v. with rate $\mu(k-(n-1))$ (Hint: at the end of a swapping period there are {\em at most} $n-1$ busy links so that the next swapping period will not occur before $n$ links become busy; this
duration is lower bounded by an exponential r.v. with rate $\mu(k-(n-1))$).

At time $t'_j$, the  state of the system when $\Delta=0$ (i.e. $X(t'_j)$) and the state of the system when $\Delta>0$ are the same. Therefore, the systems when
$\Delta=0$ and $\Delta>0$ couple infinitely often (i.e. at times $\{t_j\}$) , from which we may conclude  both systems have the same stability condition, namely, $n<k$ as shown
in Section \ref{subsec:stability} for $\Delta=0$. 


